NOAHQA: Numerical Reasoning with Interpretable Graph Question Answering Dataset

While diverse question answering (QA) datasets have been proposed and contributed significantly to the development of deep learning models for QA tasks, the existing datasets fall short in two aspects. First, we lack QA datasets covering complex questions that involve answers as well as the reasoning processes to get the answers. As a result, the state-of-the-art QA research on numerical reasoning still focuses on simple calculations and does not provide the mathematical expressions or evidences justifying the answers. Second, the QA community has contributed much effort to improving the interpretability of QA models. However, these models fail to explicitly show the reasoning process, such as the evidence order for reasoning and the interactions between different pieces of evidence. To address the above shortcomings, we introduce NOAHQA, a conversational and bilingual QA dataset with questions requiring numerical reasoning with compound mathematical expressions. With NOAHQA, we develop an interpretable reasoning graph as well as the appropriate evaluation metric to measure the answer quality. We evaluate the state-of-the-art QA models trained using existing QA datasets on NOAHQA and show that the best among them can only achieve 55.5 exact match scores, while the human performance is 89.7. We also present a new QA model for generating a reasoning graph where the reasoning graph metric still has a large gap compared with that of humans, e.g., 28 scores.

==> acl-ijcnlp2021-templates/section/1_intro_old.tex <==


\section{Introduction}
%##### begin of another version ####
Mathematics plays a fundamental role in modern Science and is one of the clearest exponents of the creative power of the human mind~\cite{vazquez2001importance}.
To maker artificial intelligence come back to basics for improving Mathematics is essential for not only modern Science but also real life.
Although it is still far from pushing Mathematics research, we would like to go for a further step to let machines better understand the real problems of applying simple Mathematics.
In this work, we will focus on labeling a conversational dataset for answering math word questions.

\begin{figure}[!t]
 \centering
    \includegraphics[width=0.44\textwidth]{acl-ijcnlp2021-templates/image/example.pdf}
    \caption{A data example.}
    \label{fig:example}
\end{figure}

\input{acl-ijcnlp2021-templates/table/data_comparison}
Math word question answering (QA) dataset~\cite{Ling2017ProgramIB} was firstly formulated into a multi-choice QA problem by selecting a correct answer from given candidates  for answering a math question in text. 
Although rationales behind the questions are given, their descriptions in text are not in a good format and harder for machines to understand.
Later on, clearer arithmetic expressions for solving questions are further annotated to build the MathQA dataset~\cite{Amini2019MathQATI}.
However, the alignments of sub-expressions and the corresponding text segments are still un-labelled, thus it is still challenging to smoothly convert questions into expressions.

How to let the models learn reasoning process is one of the key components of solving matching word questions. Recently, a large number of QA datasets for reasoning show up to the community. For example, Multi-hop QA datasets, including HotpotQA~\cite{yang2018hotpotqa}, $\mathrm{R^4C}$~\cite{inoue2020r4c}, and 2WikiMultiHopQA~\cite{ho2020constructing}, target on training models to learn reasoning across paragraphs.  DropQA~\cite{dua2019drop} and Dream~\cite{sun2019dream} target on learning multi-step compositional and discrete reasoning. Conversational QA~\cite{reddy2019coqa} is to make models understand the rationale under conversations.


Inspired by these reasoning datasets, especially conversational QA~\cite{reddy2019coqa} and multi-hop QA~\cite{yang2018hotpotqa}, we would like to construct a new math word dataset that can decompose hard math word questions into simpler ones. The simpler questions can be progressively generated by annotators in a format of conversation, an example of which is shown in Figure~\ref{fig:example}. Moreover, when labeling the answers, we also require the annotators to label the evidence directly leading to the answer. Thus more reasoning supervision is introduced and a labeled reasoning process graph can be constructed as shown in Figure~\ref{fig:example}. Finally, to draw more attention from different communities, we also provide the dataset in both Chinese and English for cross-lingual research. A comparison of the differences between our dataset and others is shown in Table~\ref{tab:data_comparison}.

To produce the reasoning process graph while answering questions, we propose the Reasoning Process Graph-QANet (\model) model, including a graph reasoning module with edge classification, as our baseline model. We additionally apply strong baselines from the other four datasets, i.e., CoQA, HotpotQA, Math23K, and DropQA, on our \dataset~dataset. Furthermore, we introduce an automatic evaluation method named $\mathrm{DAG}_{sim}$, considering the structural and semantic similarity at the same time between the predicted and ground-truth reasoning process graphs. Experiments show that the best model \model~is still $27.98$ and $29.82$ exact match scores behind humans for answers and $28.01$ and $18.14$ $\mathrm{DAG}_{sim}$ scores behind human for reasoning process graph on the English and Chinese versions of \dataset, respectively. It indicates our dataset can strongly support future research on multi-step complex reasoning and its explainability.

% *********

%##### end of another version ####

% Question Answering (QA) represents a core set of natural language understanding tasks to develop intelligent systems that can read, reason, and answer questions. Despite the many diverse QA datasets, \eg, span-extraction~\citep{rajpurkar2016squad}, multiple-choice~\citep{lai2017race} and open-domain~\citep{kwiatkowski2019natural}, most of them involve QA tasks that neither require explaining how to obtain answers nor answering complex questions. 
% \begin{figure}[!t]
%  \centering
%     \includegraphics[width=0.47\textwidth]{acl-ijcnlp2021-templates/image/example.pdf}
%     \caption{A data example.}
%     \label{fig:example}
% \end{figure}

% On the one hand, {\color{red}Some existing datasets with rationales as supervision information for explaining the predictions}, such as CoQA~\cite{reddy2019coqa}, do not require models to perform multi-hop reasoning. Multi-hop QA datasets, such as HotpotQA~\cite{yang2018hotpotqa}, $\mathrm{R^4C}$~\cite{inoue2020r4c}, and 2WikiMultiHopQA~\cite{ho2020constructing}, include paragraphs connected through hyperlinks from one Wikipedia article to another. They tend to find evidence step by step, so the reasoning process is more like a reasoning chain, which is not suitable for compositional and discrete reasoning.

% On the other hand, QA datasets, which support QA tasks with multi-step compositional and discrete reasoning, such as DropQA~\cite{dua2019drop} and Dream~\cite{sun2019dream}, have no annotations of the reasoning process. Although math word question answering dataset MathQA~\cite{Amini2019MathQATI} has annotations of arithmetic expressions, we still are unsure which text segments contribute to the predicted sub-expressions.



% To address the limitations of existing benchmarks, we present a new conversational math word question answering a dataset named \dataset, requiring multi-step compositional and discrete reasoning to measure machines’ ability to generate a correct reasoning process graph while answering a question correctly.  
% % Image a scenario in an elementary school mathematics lesson. The teacher is guiding students to solve a math word problem (MWP) by interactive communication. They first find the relevant evidence in the problem description, compose a simple sub arithmetic expression, and then compose a more extended arithmetic expression. This progress will not end until the final answer is obtained. 
% As shown in Figure~\ref{fig:example}, each example consists of a given MWP as the paragraph, a QA style conversation, and first-order evidence to support to answer each question. One first-order evidence is either text segment in the given paragraph or history QA pair. We can construct the reasoning process graph for each question by visiting first-order evidence recursively. 

% To build this dataset, We firstly extract paragraphs from two existing MWP datasets, i.e., Math23K and MAWPS. secondly, annotators create conversations in Chinese and label the evidence. Lastly, we translate the dataset into English by Google translation and correct the annotation and translation errors. Finally, We construct a Chinese and a paired English version for CoMWQA. Each version includes around 100k question answering pairs in the multi-turn conversation.

% To produce the reasoning process graph while answering the question, we propose the Reasoning Process Graph-QANet (RPG-QANet) model, including a graph reasoning module with edge classification, as our baseline model. We additionally apply strong baselines from the other four datasets, i.e., CoQA, HotpotQA, Math23K, and DropQA, on our \dataset~ dataset. Furthermore, we introduce an automatic evaluation method named $\mathrm{DAG}_{sim}$, considering the structural and semantic similarity at the same time between the predicted and ground-truth reasoning process graphs. Experiments show that the best model RPG-QANet is still $34.54$ and $29.82$ exact match scores behind humans for answers and xx, xx $\mathrm{DAG}_{sim}$ scores behind human for reasoning process graph on the English and Chinese versions of \dataset, respectively. It indicates our dataset can strongly support future research on multi-step complex reasoning and its explainability.

%\input{acl-ijcnlp2021-templates/table/1_appendix}




==> acl-ijcnlp2021-templates/section/3_data_collection_old.tex <==

\section{Data Collection }

In this section, we describe the collection process of \dataset. 
First, we extract passages from two existing math word problem datasets Math23K and MAWPS. Second, conversations in Chinese are created by crowdsourcing. We then get annotators to label the evidence, and translate the dataset into English by Google Translation. Finally, we manually correct the annotation and translation errors. We elaborate each step as follows.

\noindent\textbf{Raw Passages Preparation.}
A math word problem (MWP) is composed of a short passage and a question that naturally requires the model to carefully understand the passage and take a few steps to solve. We collect questions from two classical open-source MWP datasets: the Chinese word problem dataset Math23K~\cite{Wang2017DeepNS} and the English word problem dataset MAWPS~\cite{KoncelKedziorski2016MAWPSAM}.  
We curated $19,098$ MWPs from Math23K and $2,249$ MWPs from MAWPS. 

% We selected $19,098$ MWPs from Math23K and $2,249$ MWPs from MAWPS as the starting points for conversations. 

\noindent\textbf{Conversation Construction.}
To construct conversations that meet the requirement of multi-step reasoning for solving complex questions,
%, we first automatically split the original MWPs into background passages and questions. Given the stories as passages, 
we treat the original questions in MWPs as references to guide a group of undergraduate students as annotators in asking and answering questions step by step from easy to difficult.
% To avoid the questions to be narrowly defined, 
To diversify types of questions, we pre-define six types of question-answer pairs (i.e., ``Extraction'', ``Numerical Reasoning'', ``Counterfactual'', ``Comparison'', ``Yes/No'', and ``Unanswerable'') and present examples of predefined types to encourage annotators to create diverse questions.
%To ensure the length of conversation turns and analyze data further, 
We require annotators to provide at least five conversation turns for each passage and mark the types of question-answer pairs for further analysis. 
Since the crowd workers contributed the conversations in Chinese, we translate the passages from MAWPS to Chinese using Google Translation. %All the annotated conversations are in Chinese.

\noindent\textbf{Evidence Labeling and Translation.}
We recruit another group of undergraduates to label the evidence for each turn.  Annotators start with the first turn and label the spans from the passage or question-answer pairs in previous turns as evidence, which directly supports the answer of the current question. This process is repeated until the evidence of the last turn is labeled.
During evidence labeling, annotators mark the question-answer pair as incorrect once they find that the answer is not right. 
Meanwhile, we translate the passages and annotated conversations into English by Google Translation.

\noindent\textbf{Error Correction.}
To obtain a higher quality English dataset, we invite a group of graduates with English Translation as their major to review the translated annotations and to correct grammatical and pragmatic errors in the text. Morover, we manually correct the wrong answers marked by annotators during evidence labeling. Finally, we obtain a high-quality Chinese dataset and a moderate-quality paired English translated dataset.

==> cover_letter.tex <==
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[]{emnlp2021}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{epstopdf}
% \usepackage{array}
% \usepackage{pgfplots}
% \usepackage{wrapfig}

% \usepackage{amsmath}

% \usepackage{pifont} 
% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}%

% \usepackage{url}
% \usepackage{xcolor}
% \usepackage{setspace}
% \newcommand{\shuo}[1]{\textcolor{blue}{\small{\bf [Shuo: #1 ]}}}
% \input{acl-ijcnlp2021-templates/commands}
% \newcommand{\zqy}[1]{\textcolor{red}{#1}}
% \makeatletter
% \newcommand{\printfnsymbol}[1]{%
%   \textsuperscript{\@fnsymbol{#1}}%
% }
% \makeatother

% \title{\dataset: Numerical Reasoning with Interpretable Graph Question Answering Dataset \\ \textit{Cover Letter}}

% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row" of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% % \author{
% %   Paper ID 3718
% % }

% \begin{document}
% % \thanks{*These authors contributed equally.}

% \maketitle


% \section{Ethics Concerning}
% \begin{figure*}[h!]
%  \centering
%     \includegraphics[width=1\textwidth]{acl-ijcnlp2021-templates/image/salary.pdf}
%     \caption{The detailed minimum wage in Province Sichuan of China.}
%     \vspace{-0.56cm}
%     % \vspace{-1px}
%     \label{fig:salary}
% \end{figure*}
% We thank the ethical reviewer for the comments. We have added details about our worker compensation in Section 9 "Ethics" of the paper. Specifically, we recruited 30 annotators from the Chinese universities. We paid them CNY1400 per 1000 samples. On average, it took 83.33 hours to annotate 1000 samples. So the hourly salary worked out to be around CNY16.8 per hour, which is equivalent to USD2.52 per hour  (according to the average exchange rate of CNY to USD in 2018: 1 USD = 6.6118 CNY). As we showed in Figure~\ref{fig:salary}, please note that the average minimum hourly wage in the Sichuan Province of China (\url{https://en.wikipedia.org/wiki/Minimum_wage_in_China}) is CNY16.3 per hour in 2018. Therefore, our pay is slightly above the average minimum hourly wage. In total, we spent USD4500 in this dataset.


% \section{Changes from EMNLP submission}
% Overall, we highlighted the dataset quality issues and ethics concerning of our dataset. In this updated version, we mainly revised three parts: (1) giving more detailed descriptions of data collection process; (2) adding more experiments to prove the quality of dataset, e.g. necessity of passages and historical QA pairs; (3) giving a detailed explanation of ethics concern.

% \noindent \textbf{Introduction.} We corrected the previous typos in Figure 1 of the revised paper. 

% \noindent \textbf{Task (Section 2).} We further explained the advantages of our proposed reasoning graph evaluation method, $\mathrm{DAG}_{sim}$, over other traditional graph similarity evaluation.

% \noindent \textbf{Data Collection (Section 3).} (1) We highlighted the benefit of adapting questions in original MWPs as the reference to guide annotators to create conversations. (2) We described the specific procedure of "quality control mechanism of quantitative sampling" more clearly. (3) We supplemented the process of how we evaluated the samples to get Cohen’s kappa scores.

% \noindent \textbf{Experiment (Section 6).} (1) In the beginning, we added the descriptions of how to calculate human judgment scores for answers and reasoning graphs to "Baselines" in subsection "Experimental Settings". (2) We added the statistical significance measures, p-value, for the main results in subsection "Results and Discussion". (3) In the subsection "Results and Discussion", we added a specific analysis in "Analysis of the Necessity of Passages and Historical QA Pairs", as shown in Table 7, where we compare the experimental results on the condition of masking passage or history content respectively, indicating that passage  or  history content  is  indispensable  to  predict  answers and evidence. 

% \noindent \textbf{Related Work (Section 7).} (1) We updated the relevant references to the "Math Word Problem" domain. (2) We added references to the "Interpretable Reasoning", including previous missing references.

% \noindent \textbf{Ethics (Section 9).} In this new section, we focus on clarifying the cost of annotating the dataset and the Ethics Concerning relating to the hourly wage paid to the annotator.

% \noindent \textbf{Appendix.} Firstly, we added a new section, Interface of Conversation Collection, to show the translated interface of conversation annotation. Meanwhile, we modified the presentation form of the reasoning graph in Figure 8 to make it consistent with the form of reasoning graph in Figure 1 of the revised paper.



% \section{Response to Reviews.}
% \textbf{\color{red}{Strength from R1:}} explainable QA with the reasoning graph setting is novel. The difference is well illustrated in Figure 2. I think that this is an important problem that needs to be addressed in explainable QA.
% \\

% \noindent\textbf{\color{blue}{R1Q1:}} it is unclear how the quality of the annotated dataset is ensured. The paper says "for every 100 sets of conversation generated, we checked 20 randomly selected sets.", but it does not mention how the evaluation result was.

% \noindent\textbf{\color{blue}{Response:}} when we found any error in the sampled generated conversation, we requested the corresponding annotator to review all his annotations in the 100 sets of conversation again. We will elaborate more on this in the revised version. In addition, to ensure the quality of the annotated dataset, annotators in the evidence labeling phase mark incorrect QA pairs once they found the answers are incorrect. Annotators in the error correction phase correct marked incorrect QA pairs and translation errors. Finally, two annotators try to answer 300 randomly selected examples and mark them as valid or invalid. Cohen’s score reflects inter-annotator agreement was good.

% \noindent\textbf{\color{blue}{Remark:}}
% we have added this content in Section "Data Collection": "Once any error was... s 100 samples of conversation."
% \\

% \noindent\textbf{\color{blue}{R1Q2:}} though the dataset is described as an instance of an explainable QA task, I feel the gap between its goal and the dataset construction process (Sec. 3). According to Sec. 3, the annotators come up with multiple questions independently and the relation between these questions is annotated later, which will be a reasoning graph here. I'm not sure that these related (sub)questions can serve as a reasoning process illustrated in Figure 2.

% \noindent\textbf{\color{blue}{Response:}} sorry for the confusion. In our construction process, we assigned one conversation set to one annotator. In addition, questions in the original MWPs usually require multi-step calculation to solve. For a conversation data example, we also use the question in the original MWP as the reference to guide an annotator to create QA pairs, which helps enhance relations between QA pairs in the conversation.

% \noindent\textbf{\color{blue}{Remark:}}
% We clarified this confusion in Section 3 “Data Collection”: "It helps to enhance... in the conversation".
% \\

% \noindent\textbf{\color{blue}{R1Q3:}} Typos, "L093: to some extend => to some extent", "L226: the work, The guidelines => the work. The guidelines".

% \noindent\textbf{\color{blue}{Response:}} thanks for pointing these out.  We will carefully proofread the paper.

% \noindent\textbf{\color{blue}{Remark:}} 
% we have corrected these typos in Section "Introduction" and "Data Collection".
% \\

% \noindent\textbf{\color{red}{Strength from R2:}}
% 1. A substantial paper with a new dataset, model, and metric. All three would be helpful in the community.
% 2.  Lots of analysis and experiments.
% \\

% \noindent\textbf{\color{blue}{R2Q1:}} it is not clear how the $\mathrm{DAG}_{sim}$ metric correlates with human judgment. Moreover, in Table 5 what does the human score refers to. What are the human judgment scores? How does this metric co-relate to other earlier graph/sub-graph similarity metrics? How is this metric better than a simple Precision-Recall of the expected Edges? 

% \noindent\textbf{\color{blue}{Response:}} (1) For "$\mathrm{DAG}_{sim}$": Good question! Human judgment is prone to giving a binary measure instead of a gray-scale measure. The proposed $\mathrm{DAG}_{sim}$ calculates a score ranging from 0 to 1 to measure the similarity between two graphs. 
% Most of traditional graph similarity methods, e.g., Graph Edit Distance (GED), are hard to scale and ignore the semantic similarity between two nodes (two text nodes as 1 if exact matching, 0 otherwise). $\mathrm{DAG}_{sim}$ can run efficiently and consider structured and semantic similarity simultaneously. 
% Precision-recall of the expected edges is a good evaluation metric considering edges and nodes. However, it ignores the semantic similarity of two text nodes. Thus, we think the proposed $\mathrm{DAG}_{sim}$ is more comprehensive; (2) For "Human judgment scores": Sorry for the missing content of how to calculate human judgment scores (Different from human judgment mentioned in "$\mathrm{DAG}_{sim}$") in the paper. To establish human performance for answers and reasoning graphs, we first randomly sampled 300 examples from the test set. We then had two annotators to predict answers and their corresponding reasoning graphs for these examples. For each example, we average exact match scores as evaluation for two predicted answers, and exact match scores and "$\mathrm{DAG}_{sim}$" scores for two predicted graphs.

% \noindent\textbf{\color{blue}{Remark:}} (1) for "$\mathrm{DAG}_{sim}$": at the end of Section "Task",  we further explained the advantages of "$\mathrm{DAG}_{sim}$": "Most  of  traditional  graph... semantic similarity simultaneously."; (2) for "Human judgment scores": we added this part to "Baselines" in Section 6.1 "Experimental Settings".
% \\

% \noindent\textbf{\color{blue}{R2Q2:}} dataset is bilingual, with both Chinese and English conversations and QA pairs. However, the English text is generated with Google Translate and corrected by English Translation major graduates. The corrections were verified for 300 samples only. Similarly, other annotator agreement scores, details about the number of annotators and the pay is absent.

% \noindent\textbf{\color{blue}{Response:}} for correction and agreement scores, please also kindly refer to R1Q1. 
% For annotator details, we had 23 undergraduates, 4 undergraduates, and 3 graduates majoring in English for conversation collection, error correction, evidence labeling and translation. The total cost is about 4500 US dollars.

% \noindent\textbf{\color{blue}{Remark:}} we clarified a detailed number of annotators in "annotation de-biasing" in Section3 “Data Collection”, then the "total cost" is added in further detail in Section "Ethics".
% \\

% \noindent\textbf{\color{blue}{R2Q3:}} the proposed model extends the NumNet, NAQANet, with an additional reasoning graph generation module. Direct comparison to current methods is a bit unfair, as they lack the additional supervision and inductive bias the reasoning graph generation module provides. Similarly, the comparison on the new proposed dataset for zero-shot evaluation is a bit unfair. However, it would be interesting to observe how training on NoahQA, the models perform on other datasets in zero/few-shot setting.

% \noindent\textbf{\color{blue}{Response:}} Comparison to current methods. Please kindly refer to the ablative settings in Table 4, where we remove the additional supervision and inductive bias provided by the reasoning graph generation module (w/o Edge and w/o GCN). We also highlight that our main contribution is the novel \dataset{}. The proposed model only provides a baseline to facilitate future research.
% \\

% \noindent\textbf{\color{blue}{R2Q4:}} lack of statistical significance measures. 

% \noindent\textbf{\color{blue}{Response:}} Thanks for the suggestion. We perform the one-sample t-test, and p-value = 2e-6 < 0.05 indicates that the improvements of RGNet w/o Edge over FlowQA (the strongest baseline) are statistically significant.

% \noindent\textbf{\color{blue}{Remark:}} we explained this problem in Section6.2 "main results", "We also perform the one-sample...are statistically significant".
% \\

% \noindent\textbf{\color{blue}{R2Q5:}} missing References: some work similar to the reasoning graph generation but on a different domain.

% \noindent\textbf{\color{blue}{Response:}} thanks for indicating the missing reference, we will add it in the revised version.

% \noindent\textbf{\color{blue}{Remark:}} we have added them to "Interpretable Reasoning" in Section 7 “Related work”.
% \\

% \noindent\textbf{\color{red}{Strength from R3:}}
% 1. The proposed dataset brings complex numerical, multihop and conversational reasoning together with addition of interpretable evidences. Researchers working on multihop reasoning and model interpretability should find this useful.
% 2. The dataset seems challenging for existing models and so can potential spur modeling advances.
% 3. The paper is clearly written and easy to understand.
% \\

% \noindent\textbf{\color{blue}{R3Q1:}} information about Human scores is missing.

% \noindent\textbf{\color{blue}{Response:}} please kindly refer to R1Q1 and R2Q2 for details.
% \\

% \noindent\textbf{\color{blue}{R3Q2:}} it's unclear how cheatable/gamble this dataset is.
% Several previous works have shown that multihop reasoning and conversational datasets have artifacts that allow them to be cheated with superficial patterns and no multihop reasoning. From the experiments shown though, I can't tell if that isn't the case here.
% If nothing else, there should have been some input ablation experiments like 1. mask out paragraph content and see how predictable answer+evidence is 2. for $\mathrm{Q}_{i}$, mask out question content for all questions except $\mathrm{Q}_{i}$ and see how predictable answer+evidence is.

% \noindent\textbf{\color{blue}{Response:}} thanks for the suggestion! We conduct the experiment as follows, EM scores for answer and reasoning graph (evidence) of zh test set in w/o passage content setting drop from 62.94 to 19.31 and from 59.32 to 9.01 respectively. In addition, EM scores of span and arithmetic answers drop significantly, from 73.20 to 1.12 and from 33.73 to 11.79. EM scores for answer and reasoning graph of zh test set in w/o history content setting drops to 52.67 and to 38.92 respectively. In addition, EM scores of arithmetic answers drop most, from 33.73 to 23.68. These results indicate that passage or history content is indispensable to predict answers and evidence.

% \noindent\textbf{\color{blue}{Remark:}} we added a subsection "Analysis of the Necessity of Passages and Historical QA Pairs" in Section 6.2 to specifically analyze this problem and show the experimental table.
% \\

% \noindent\textbf{\color{blue}{R3Q3:}} it's be useful to share what annotation interfaces look like, perhaps in the appendix.

% \noindent\textbf{\color{blue}{Response:}} we use excel as the annotation interface. We also provide annotation guidelines (described in Section 3) and we will share the annotation interfaces in the revised version.

% \noindent\textbf{\color{blue}{Remark:}} we added a subsection “interface of Conversation Collection” to show our annotation interface in the "Appendix". The original content of the annotation interface is Chinese, and we show the translated version.
% \\

% \noindent\textbf{\color{blue}{R3Q4:}} in experiment, what is pretraining referring to? Does it mean whether to use pretrained Roberta/XLM-R or randomly initialized one?

% \noindent\textbf{\color{blue}{Response:}} yes, pretraining refers to the usage of the pretraining language model Roberta~\cite{liu2019roberta}/XLM-R~\cite{conneau-etal-2020-unsupervised}.

% \noindent\textbf{\color{blue}{Remark:}} we clarified the fuzzy reference of "pretraining"  in Table 4 and "Implementation Details" in Section 6 "Experiment".
% \\

% \noindent\textbf{\color{blue}{R3Q5:}} I'm assuming table 4 is representing answer EMs. It'd be good to mention is in the table title or caption.

% \noindent\textbf{\color{blue}{Response:}} sorry for the confusion, EM in table 4 denotes the answer EM score and EM in table 5 denotes the reasoning graph EM score. We will enhance the writing in the revised version.

% \noindent\textbf{\color{blue}{Remark:}} For the confusion of the same word "EM" in the two experimental tables, we make a distinction in the “Main Results” and "Reasoning Graph Evaluation" in section 6.2 "Results and Discussion", particularly, we denote "GEM" as Exact Match for reasoning graphs. Also, we mention the EM score for reasoning graphs in Table 5.
% \\

% \noindent\textbf{\color{blue}{Meta-Review Q1:}}  Q7 in figure 1 of the paper is both ungrammatical and appears to have the wrong answer.

% \noindent\textbf{\color{blue}{Response:}} really sorry for the typos. The original data is correct and we already performed the proofreading in the camera-ready version.

% \noindent\textbf{\color{blue}{Remark:}} we have corrected this typos in Figure 1 of the revised paper, specifically, we added the missing word "until" in the "Q7" and corrected "A7".
% \\

% \noindent\textbf{\color{blue}{Meta-Review Q2:}} Q4 in the top of Figure 8 does not need Q2 or Q3, as Q4 is a self-contained question.

% \noindent\textbf{\color{blue}{Response:}} Q4 isn't self-contained question. Q4 is “Did bookstore sell more in the  morning or in the afternoon?”, Q2,Q3 provide the specific coreference which is needed in Q4 to compare.
% \\

% \noindent\textbf{\color{blue}{Meta-Review Q3:}} the answer to Q7 in the top of Figure 8 has a reference to A6; is this actually expected to be output by the system? If so, why? The fact that exact string match is used for evaluation, with a generative model outputting token strings, is concerning to me, especially with unanswered questions about exactly how those strings are formatted.

% \noindent\textbf{\color{blue}{Response:}} as we mentioned in Section 2 "Task", "we only use exact match (EM) score as our evaluation metric for answer correctness". Especially for Arithmetic problems, we generated an equation and evaluated the calculated answer of the equation. For A7 in above example of Figure 8, we need to generate [A6] token, and then calculated the equation where we replaced the token [A6] with string of previous A6 during the evaluation process.
% \\
% % Entries for the entire Anthology, followed by custom entries
% \bibliography{coverletter}
% \bibliographystyle{acl_natbib}


% \end{document}

